enpheeph: A Fault Injection Framework for Spiking and Compressed Deep Neural Networks

Research on Deep Neural Networks (DNNs) has focused on improving performance and accuracy for real-world deployments, leading to new models, such as Spiking Neural Networks (SNNs), and optimization techniques, e.g., quantization and pruning for compressed networks. However, the deployment of these innovative models and optimization techniques introduces possible reliability issues, which is a pillar for DNNs to be widely used in safety-critical applications, e.g., autonomous driving. Moreover, scaling technology nodes have the associated risk of multiple faults happening at the same time, a possibility not addressed in state-of-the-art resiliency analyses. Towards better reliability analysis for DNNs, we present enpheeph, a Fault Injection Framework for Spiking and Compressed DNNs. The enpheeph framework enables optimized execution on specialized hardware devices, e.g., GPUs, while providing complete customizability to investigate different fault models, emulating various reliability constraints and use-cases. Hence, the faults can be executed on SNNs as well as compressed networks with minimal-to-none modifications to the underlying code, a feat that is not achievable by other state-of-the-art tools. To evaluate our enpheeph framework, we analyze the resiliency of different DNN and SNN models, with different compression techniques. By injecting a random and increasing number of faults, we show that DNNs can show a reduction in accuracy with a fault rate as low as 7 x 10 ^ (-7) faults per parameter, with an accuracy drop higher than 40%. Run-time overhead when executing enpheeph is less than 20% of the baseline execution time when executing 100 000 faults concurrently, at least 10x lower than state-of-the-art frameworks, making enpheeph future-proof for complex fault injection scenarios. We release enpheeph at https://github.com/Alexei95/enpheeph.

==> content/paper/sections/0_round0.tex <==
\section{Round 0}


\textbf{Idea:} Fault Injection Framework for compressed and spiking neural networks


\textbf{Novel contributions:}
\begin{itemize}
    \item bit-level exact fault injection on GPU/CPU, with support for other devices/accelerators, fully customizable for efficiency/depth of saved information
    \item comparison with existing frameworks, providing full reproducibility of the experiments
\end{itemize}


\textbf{Scientific Challenges:}
\begin{itemize}
    \item 
    \item 
    \item 
\end{itemize}

\textbf{Current Results:}
\begin{itemize}
    \item Much faster than state-of-the-art
    \item Similar accuracy/fault coverage as state-of-the-art
\end{itemize}

\textbf{Comparison with SotA:}
\begin{itemize}
    \item All the comparisons from the README
\end{itemize}

\textbf{Expected Results:}
\begin{itemize}
    \item initial resiliency for pruned/quantized/spiking models
    \item 
\end{itemize}

